Coopetitive Soft Gating Ensemble

In this article, we propose the Coopetititve Soft Gating Ensemble or CSGE for general machine learning tasks and interwoven systems. The goal of machine learning is to create models that generalize well for unknown datasets. Often, however, the problems are too complex to be solved with a single model, so several models are combined. Similar, Autonomic Computing requires the integration of different systems. Here, especially, the local, temporal online evaluation and the resulting (re-)weighting scheme of the CSGE makes the approach highly applicable for self-improving system integrations. To achieve the best potential performance the CSGE can be optimized according to arbitrary loss functions making it accessible for a broader range of problems. We introduce a novel training procedure including a hyper-parameter initialisation at its heart. We show that the CSGE approach reaches state-of-the-art performance for both classification and regression tasks. Further on, the CSGE provides a human-readable quantification on the influence of all base estimators employing the three weighting aspects. Moreover, we provide a scikit-learn compatible implementation.

==> chapters/ausblick.tex <==
\section{Ausblick}
\label{sec:ausblick}

Dieser Abschnitt gibt einen Ausblick auf mögliche Erweiterungen Ihrer Arbeit. Erläuteren Sie auch an dieser Stelle, welche Schwierigkeiten sich bei der Bearbeitung ihres Themas ergaben. Was hätte man besser, anderst machen können? Was sollte zusätzlich noch gemacht / untersucht werden? Vielleicht konnten aus zeitlichen Gründen nicht mehr alle Ideen durchgeführt werden. 

==> chapters/titlepage.tex <==
%
% Diplomarbeit mit LaTeX
% ===========================================================================
% This is part of the book "Diplomarbeit mit LaTeX".
% Copyright (c) 2002-2005,2007 Tobias Erbsland
% Copyright (c) 2005 Andreas Nitsch
% See the file diplomarbeit_mit_latex.tex for copying conditions.
%

\begin{titlepage}
    \begin{center}
    
		\begin{figure}
				\includegraphics[width=0.35\textwidth]{images/uni-logo}
				\hfill
				\includegraphics[width=0.35\textwidth]{images/ies-logo}
		\end{figure}

    \vspace*{0.5cm}

    \large{Department Electrical Engineering / Computer Science}\\
    \vspace*{0.5cm} \large{Department Intelligent Embedded Systems (IES)\\Prof. Dr. Bernhard Sick}

    \vspace*{2cm}
 		% BITTE EINES DER BEIDEN WÄHLEN!! %
    \large {PROJECT REPORT}\\
    \vspace*{1cm} \Huge {\textbf{Coopetitive Soft Gating Ensembles} }\\
    \vspace*{1cm}

    \normalsize{submitted by} \\
    \large{Stephan Deist} \\
    \vspace*{1.5cm} \normalsize{\today}

    \vspace*{1cm}

        \begin{center}
            \begin{tabular}{ll}
             Advisor: Maarten Bieshaar and Jens Schreiber
            \end{tabular}
        \end{center}

    \end{center}
\end{titlepage}

